Neural Network Based Reinforcement Learning for Audio-Visual Gaze Control in Human-Robot Interaction

This paper introduces a novel neural network-based reinforcement learning approach for robot gaze control. Our approach enables a robot to learn and to adapt its gaze control strategy for human-robot interaction neither with the use of external sensors nor with human supervision. The robot learns to focus its attention onto groups of people from its own audio-visual experiences, independently of the number of people, of their positions and of their physical appearances. In particular, we use a recurrent neural network architecture in combination with Q-learning to find an optimal action-selection policy; we pre-train the network using a simulated environment that mimics realistic scenarios that involve speaking/silent participants, thus avoiding the need of tedious sessions of a robot interacting with people. Our experimental evaluation suggests that the proposed method is robust against parameter estimation, i.e. the parameter values yielded by the method do not have a decisive impact on the performance. The best results are obtained when both audio and visual information is jointly used. Experiments with the Nao robot indicate that our framework is a step forward towards the autonomous learning of socially acceptable gaze behavior.

==> inkscapeInclude.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbold}

% definition de macros pour les equations mathematiques

% definitions de Gabriella

\def\eq#1{(\ref{#1})}
\def\pmb#1{\setbox0=\hbox{#1}%
  \kern-.02em\copy0\kern-\wd0
  \kern-.035em\copy0\kern-\wd0
  \kern-.02em\raise.03em\box0 }

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newcommand{\matx}[1]{\mbox{\bf $#1$}}
\newcommand{\vect}[1]{\mbox{{\boldmath $#1$}}}
\newcommand{\ovec}[1]{\overline{\vect{#1}}}
\newcommand{\overmat}[1]{\overline{\matx{#1}}}
\newcommand{\hatmat}[1]{\hat{\matx{#1}}}
\newcommand{\hatvec}[1]{\hat{\vect{#1}}}

\newcommand{\mm}[1]{\mbox{\bf $#1$}}
\newcommand{\vv}[1]{\mbox{{\boldmath $#1$}}}
\newcommand{\cc}[1]{{\cal{#1}}}
 
\newcommand{\ovv}[1]{\overline{\vv{#1}}}
\newcommand{\omm}[1]{\overline{\mm{#1}}}
\newcommand{\occ}[1]{\overline{\cal{#1}}}
 
\newcommand{\tvv}[1]{\widetilde{\vv{#1}}}
\newcommand{\tmm}[1]{\widetilde{\mm{#1}}}
\newcommand{\tcc}[1]{\widetilde{\cal{#1}}}
 
 
\newcommand{\hvv}[1]{\widehat{\vv{#1}}}
\newcommand{\hmm}[1]{\widehat{\mm{#1}}}
\newcommand{\hcc}[1]{\widehat{\cal{#1}}}

%\newcommand{\dvv}[1]{\stackrel{\bullet}{\vv{#1}}}
%\newcommand{\dmm}[1]{\stackrel{\bullet}{\mm{#1}}}
%\newcommand{\dcc}[1]{\stackrel{\bullet}{\cal{#1}}}

\newcommand{\dvv}[1]{\dot{\vv{#1}}}
\newcommand{\dmm}[1]{\dot{\mm{#1}}}
\newcommand{\dcc}[1]{\dot{\cc{#1}}}

%\newcommand{\crp}{\times}
\newcommand{\tp}{^{\top}}
\newcommand{\prj}{\simeq}
\newcommand{\inverse}{^{-1}}
\newcommand{\tpinv}{^{-\top}}
\newcommand{\overstar}{^{\star}}
\setlength{\parskip}{\medskipamount}

\def\proof{\noindent\hspace{2em}{\it Proof: }}
\def\endproof{\hspace*{\fill}~\par\endtrivlist\unskip}

% definitions de Radu.
\def\diag{\mbox{Diag}\:}
\def\trace{\mbox{trace}\:}
\def\rank{\mbox{rank}\:}
\def\sign{\mbox{sign}\:}
\def\spec{\mbox{spec}\:}
\def\p3{\cc{P}^3}

\def\avect{\boldsymbol{a}}
\def\bvect{\boldsymbol{b}}
\def\cvect{\boldsymbol{c}}
\def\dvect{\boldsymbol{d}}
\def\evect{\boldsymbol{e}}
\def\fvect{\boldsymbol{f}}
\def\gvect{\boldsymbol{g}}
\def\hvect{\boldsymbol{h}}
\def\ivect{\boldsymbol{i}}
\def\jvect{\boldsymbol{j}}
\def\kvect{\boldsymbol{k}}
\def\lvect{\boldsymbol{l}}
\def\mvect{\boldsymbol{m}}
\def\nvect{\boldsymbol{n}}
\def\ovect{\boldsymbol{o}}
\def\pvect{\boldsymbol{p}}
\def\qvect{\boldsymbol{q}}
\def\rvect{\boldsymbol{r}}
\def\svect{\boldsymbol{s}}
\def\tvect{\boldsymbol{t}}
\def\uvect{\boldsymbol{u}}
\def\vvect{\boldsymbol{v}}
\def\wvect{\boldsymbol{w}}
\def\xvect{\boldsymbol{x}}
\def\yvect{\boldsymbol{y}}
\def\zvect{\boldsymbol{z}}

\def\Avect{\boldsymbol{A}}
\def\Bvect{\boldsymbol{B}}
\def\Cvect{\boldsymbol{C}}
\def\Dvect{\boldsymbol{D}}
\def\Evect{\boldsymbol{E}}
\def\Fvect{\boldsymbol{F}}
\def\Gvect{\boldsymbol{G}}
\def\Hvect{\boldsymbol{H}}
\def\Ivect{\boldsymbol{I}}
\def\Jvect{\boldsymbol{J}}
\def\Kvect{\boldsymbol{K}}
\def\Lvect{\boldsymbol{L}}
\def\Mvect{\boldsymbol{M}}
\def\Nvect{\boldsymbol{N}}
\def\Ovect{\boldsymbol{O}}
\def\Pvect{\boldsymbol{P}}
\def\Qvect{\boldsymbol{Q}}
\def\Rvect{\boldsymbol{R}}
\def\Svect{\boldsymbol{S}}
\def\Tvect{\boldsymbol{T}}
\def\Uvect{\boldsymbol{U}}
\def\Vvect{\boldsymbol{V}}
\def\Wvect{\boldsymbol{W}}
\def\Xvect{\boldsymbol{X}}
\def\Yvect{\boldsymbol{Y}}
\def\Zvect{\boldsymbol{Z}}

\def\onevect{\boldsymbol{1}}

\def\amat{\mbox{\bf a}}
\def\bmat{\mbox{\bf b}}
\def\cmat{\mbox{\bf c}}
\def\dmat{\mbox{\bf d}}
\def\emat{\mbox{\bf e}}
\def\fmat{\mbox{\bf f}}
\def\gmat{\mbox{\bf g}}
\def\hmat{\mbox{\bf h}}
\def\imat{\mbox{\bf i}}
\def\jmat{\mbox{\bf j}}
\def\kmat{\mbox{\bf k}}
\def\lmat{\mbox{\bf l}}
\def\mmat{\mbox{\bf m}}
\def\nmat{\mbox{\bf n}}
\def\omat{\mbox{\bf o}}
\def\pmat{\mbox{\bf p}}
\def\qmat{\mbox{\bf q}}
\def\rmat{\mbox{\bf r}}
\def\smat{\mbox{\bf s}}
\def\tmat{\mbox{\bf t}}
\def\umat{\mbox{\bf u}}
\def\vmat{\mbox{\bf v}}
\def\wmat{\mbox{\bf w}}
\def\xmat{\mbox{\bf x}}
\def\ymat{\mbox{\bf y}}
\def\zmat{\mbox{\bf z}}

\def\Amat{\mbox{\bf A}}
\def\Bmat{\mbox{\bf B}}
\def\Cmat{\mbox{\bf C}}
\def\Dmat{\mbox{\bf D}}
\def\Emat{\mbox{\bf E}}
\def\Fmat{\mbox{\bf F}}
\def\Gmat{\mbox{\bf G}}
\def\Hmat{\mbox{\bf H}}
\def\Imat{\mbox{\bf I}}
\def\Jmat{\mbox{\bf J}}
\def\Kmat{\mbox{\bf K}}
\def\Lmat{\mbox{\bf L}}
\def\Mmat{\mbox{\bf M}}
\def\Nmat{\mbox{\bf N}}
\def\Omat{\mbox{\bf O}}
\def\Pmat{\mbox{\bf P}}
\def\Qmat{\mbox{\bf Q}}
\def\Rmat{\mbox{\bf R}}
\def\Smat{\mbox{\bf S}}
\def\Tmat{\mbox{\bf T}}
\def\Umat{\mbox{\bf U}}
\def\Vmat{\mbox{\bf V}}
\def\Wmat{\mbox{\bf W}}
\def\Xmat{\mbox{\bf X}}
\def\Ymat{\mbox{\bf Y}}
\def\Zmat{\mbox{\bf Z}}

\def\Abarre{\overline{\Amat}}
\def\Cbarre{\overline{\Cmat}}
\def\Mbarre{\overline{\Mvect}}
\def\Nbarre{\overline{\Nvect}}
\def\Pbarre{\overline{\Pmat}}
\def\Qbarre{\overline{\Qmat}}

\def\zeromat{\mbox{\bf 0}}
\def\zerovect{\boldsymbol{0}}
\def\unmat{\mbox{\bf 1}}
\def\unvect{\mbox{\bf 1}}
\def\idmat{\mathbb{I}}

\def\qquat{\boldsymbol{q}}

\def\itilde{\mbox{\bf \~\i}}
\def\jtilde{\mbox{\bf \~\j}}
\def\ihat{\mbox{\bf \^\i}}
\def\jhat{\mbox{\bf \^\j}}

\def\ahat{\hat{\avect}}
\def\uhat{\hat{u}}
\def\vhat{\hat{v}}
\def\what{\hat{w}}

\def\Rcal{\cal R}
\def\Pcal{\cal P}

%\newcommand{\Reel}{I\!\!R}
\newcommand{\Reel}{\mathbb{R}}
\def\Nset{\mbox{\it I\hskip -0.177em N}}
\def\EE{\mathbb{E}}
\def\II{\mathbb{I}}
\def\dd{\mathrm{d}}
\newcommand{\inv}{^{-1}}

\def\alphavect{\boldsymbol{\alpha}}
\def\betavect{\boldsymbol{\beta}}
\def\gammavect{\boldsymbol{\gamma}}
\def\deltavect{\boldsymbol{\delta}}
\def\epsilonvect{\boldsymbol{\epsilon}}
\def\varepsilonvect{\boldsymbol{\varepsilon}}
\def\zetavect{\boldsymbol{\zeta}}
\def\etavect{\boldsymbol{\eta}}
\def\thetavect{\boldsymbol{\theta}}
\def\varthetavect{\boldsymbol{\vartheta}}
\def\gammavect{\boldsymbol{\gamma}}
\def\kappavect{\boldsymbol{\kappa}}
\def\lambdavect{\boldsymbol{\lambda}}
\def\muvect{\boldsymbol{\mu}}
\def\nuvect{\boldsymbol{\nu}}
\def\xivect{\boldsymbol{\xi}}
\def\omicronvect{\boldsymbol{o}}
\def\pivect{\boldsymbol{\pi}}
\def\varpivect{\boldsymbol{\varpi}}
\def\rhovect{\boldsymbol{\rho}}
\def\varrhovect{\boldsymbol{\varrho}}
\def\sigmavect{\boldsymbol{\sigma}}
\def\varsigmavect{\boldsymbol{\varsigma}}
\def\tauvect{\boldsymbol{\tau}}
\def\upsilonvect{\boldsymbol{\upsilon}}
\def\phivect{\boldsymbol{\phi}}
\def\varphivect{\boldsymbol{\varphi}}
\def\chivect{\boldsymbol{\chi}}
\def\psivect{\boldsymbol{\psi}}
\def\omegavect{\boldsymbol{\omega}}

\def\Gammavect{\boldsymbol{\Gamma}}
\def\Deltavect{\boldsymbol{\Delta}}
\def\Thetavect{\boldsymbol{\Theta}}
\def\Lambdavect{\boldsymbol{\Lambda}}
\def\Xivect{\boldsymbol{\Xi}}
\def\Pivect{\boldsymbol{\Pi}}
\def\Sigmavect{\boldsymbol{\Sigma}}
\def\Upsilonvect{\boldsymbol{\Upsilon}}
\def\Phivect{\boldsymbol{\Phi}}
\def\Psivect{\boldsymbol{\Psi}}
\def\Omegavect{\boldsymbol{\Omega}}

\def\alphamat{{\bf \alpha}}
\def\betamat{{\bf \beta}}
\def\gammamat{{\bf \gamma}}
\def\deltamat{{\bf \delta}}
\def\epsilonmat{{\bf \epsilon}}
\def\varepsilonmat{{\bf \varepsilon}}
\def\zetamat{{\bf \zeta}}
\def\etamat{{\bf \eta}}
\def\thetamat{{\bf \theta}}
\def\varthetamat{{\bf \vartheta}}
\def\gammamat{{\bf \gamma}}
\def\kappamat{{\bf \kappa}}
\def\lambdamat{{\bf \lambda}}
\def\mumat{{\bf \mu}}
\def\numat{{\bf \nu}}
\def\ximat{{\bf \xi}}
\def\omicronmat{{\bf o}}
\def\pimat{{\bf \pi}}
\def\varpimat{{\bf \varpi}}
\def\rhomat{{\bf \rho}}
\def\varrhomat{{\bf \varrho}}
\def\sigmamat{{\bf \sigma}}
\def\varsigmamat{{\bf \varsigma}}
\def\taumat{{\bf \tau}}
\def\upsilonmat{{\bf \upsilon}}
\def\phimat{{\bf \phi}}
\def\varphimat{{\bf \varphi}}
\def\chimat{{\bf \chi}}
\def\psimat{{\bf \psi}}
\def\omegamat{{\bf \omega}}

\def\Gammamat{{\bf \Gamma}}
\def\Deltamat{{\bf \Delta}}
\def\Thetamat{{\bf \Theta}}
\def\Lambdamat{{\bf \Lambda}}
\def\Ximat{{\bf \Xi}}
\def\Pimat{{\bf \Pi}}
\def\Sigmamat{{\bf \Sigma}}
\def\Upsilonmat{{\bf \Upsilon}}
\def\Phimat{{\bf \Phi}}
\def\Psimat{{\bf \Psi}}
\def\Omegamat{{\bf \Omega}}


\def\spc{\ \ \ \ }
\def\And{\mbox{\ \ \ and\ \ \ }}

% vector: \vector{O}{M} puts an arrow on OM. 
\newcommand{\vecteur}[2]{{\boxmaxdepth=1000pt\relax\overrightarrow{#1#2}}}

\def\normal{\mathcal{N}}
\def\uniform{\mathcal{U}}
\def\student{{\textrm{St}}}

\def\indic{\mathbb{1}}
\def\Esp{\mathbb{E}}

% \DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
% \DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

%\newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{definition}{Definition}
%\newtheorem{corollary}{Corollary}[proposition]

\newcommand{\best}[1]{$\mathbf{#1}$}
%% \def\lown{\yvect_n}
%% \def\highn{\xvect_n}
%% \def\Low{\Yvect}
%% \def\High{\Xvect}
%% \def\low{\yvect}
%% \def\high{\xvect}
%% \def\phiHW{{\phivect^{\High}_{\wvect}}}
%% \def\phihW{{\phivect^{\high}_{\wvect}}}
%% \def\phihnW{{\phivect^{\high_n}_{\wvect}}}
%% \def\phihnWi{{\phivect^{\high_n}_{\wvect^{(i)}}}}
\def\lown{\yvect_n}
\def\highn{\ivect_n}
\def\Low{\Yvect}
\def\High{\Ivect}
\def\low{\yvect}
\def\high{\ivect}
\def\phiHW{{\Xvect}}
\def\phihW{{\xvect}}
\def\phihnW{{\xvect_n}}
\def\phihnWi{{\xvect_n}}


==> observation.tex <==
\subsection{Observation Representation}
\label{sec:obs}

In this section, we describe how the observations are represented in our model. Formally, we detail how $\vvect_t$,$f_t$ $\wvect_t,\thetavect_t$ and $\sigma_t$ (realizations of the random variables $\Vvect_t$,$F_t$ $\Wvect_t$,$\Thetavect_t$ and $\Sigma_t$) are computed. Concerning the visual features, we employ the full-body pose estimator described in \cite{cao2017realtime}. It provides the locations of 18 keypoints (nose, neck, shoulders, elbows, wrists, hip, knees, ankles, eyes and ears) for each detected person.
The outputs of the pose estimator are $p_n=(k_n^j,l_n^j,s_n^j), n\in \{1..N_t\}, j\in \{1..J\} $ where  $(k_n^j,l_n^j)\in \{1..N_v\}\times \{1..M_v\}$ denotes the pixel coordinates of the $j^{th}$ joints, and $s_n^j$ is a binary value such that $s_n^j=1$ if the $j^{th}$ joint is successfully detected and $s_n^j=0$ otherwise. We can now define the visual observations $\vvect_t$ as follows:
\begin{align}
\vvect_t(k,l,j) = \left\{
\begin{array}{ll}
  1 & if~\exists n \in \{1..N_t\}, s_n^j=1,(k_n^j,l_n^j)=(k,l)\\
  0 & \text{otherwise}
\end{array}
\right.
\end{align} 
Moreover, $f_t$ is computed from the channel $j_{\text nose}$ corresponding to the nose:
\begin{align}
  f_t=\sum_{\substack{k\in\{1..N_v\} \\ l\in\{1..M_v\}}}\vvect_t(k,l,j_{\text nose})
\end{align} 


Concerning the audio features, at each time step, we use
Li et al. algorithm \cite{li2016reverberant,li2017multiple} to detect sound sources.  Similarly, to the visual features, we discretize the angle space and threshold the probability values returned by the SSL algorithm in order to estimate $\wvect_t$ .
The angles of the robot head are centered and normalized to obtain $\thetavect_t\in [0,1]^2$. Finally, $\sigma_t$ is computed similarly to $f_t$ from $\wvect_t$ and $\thetavect_t$.


%% The variable $\Sigma_t$ is computed according to:
%% \begin{align}
%% \Sigma_t = \left\{
%% \begin{array}{lll}
%%   1 & if~\exists (u,v) &\in \{1..N_a\}\times\{1..M_a\}, \Wvect_t(u,v)=1 \\
%%   & &\textrm{~and~} |\theta^p_t-\theta^{p,uv}_t| <\theta^p_{\mathcal{F}}\\
%%   & &\textrm{~and~} |\theta^y_t-\theta^{y,uv}_t| <\theta^y_{\mathcal{F}}\\
%%   0 & otherwise&
%% \end{array}
%% \right.
%% \end{align}
%% where $\theta^{p,uv}_t$ and $\theta^{y,uv}_t$ are the pitch and yaw angles corresponding to the location $(u,v)$ of $\Wvect_t$ and $\theta^p_{\mathcal{F}}$ and $\theta^y_{\mathcal{F}}$ are the vertical and horizontal angles of coverage of the field of view.

